Quantum Secure Anonymous Communication Networks

Anonymous communication networks (ACNs) enable Internet browsing in a way that prevents the accessed content from being traced back to the user. This allows a high level of privacy, protecting individuals from being tracked by advertisers or governments, for example. The Tor network, a prominent example of such a network, uses a layered encryption scheme to encapsulate data packets, using Tor nodes to obscure the routing process before the packets enter the public Internet. While Tor is capable of providing substantial privacy, its encryption relies on schemes, such as RSA and Diffie-Hellman for distributing symmetric keys, which are vulnerable to quantum computing attacks and are currently in the process of being phased out. To overcome the threat, we propose a quantum-resistant alternative to RSA and Diffie-Hellman for distributing symmetric keys, namely, quantum key distribution (QKD). Standard QKD networks depend on trusted nodes to relay keys across long distances, however, reliance on trusted nodes in the quantum network does not meet the criteria necessary for establishing a Tor circuit in the ACN. We address this issue by developing a protocol and network architecture that integrates QKD without the need for trusted nodes, thus meeting the requirements of the Tor network and creating a quantum-secure anonymous communication network.

==> biography.tex <==
% \begin{IEEEbiography}[{\includegraphics[width=0.75in,height=1.0in,clip,keepaspectratio]{biopics/saidurprofile.jpg}}]%
% {Mohammad Saidur Rahman}
% is a Ph.D. Intern at the Cisco Quantum Lab and a Ph.D. Candidate in Computing and Information Sciences at Rochester Institute of Technology (RIT). His research interest is in the intersection of machine learning, security, privacy, and quantum network. 
% %He is affiliated with the Department of Computing Security and the ESL Global Cybersecurity Institute (GCI) at RIT. 
% He received his M.S. degree from the Department of Cybersecurity at RIT. He received his Bachelor's degree from the Department of Management Information Systems at the University of Dhaka, Bangladesh.
% \end{IEEEbiography}



\begin{IEEEbiographynophoto}{Mohammad Saidur Rahman}
is a Ph.D. Intern at the Cisco Quantum Lab and a Ph.D. Candidate in Computing and Information Sciences at Rochester Institute of Technology (RIT). His research interest is in the intersection of security, privacy, machine learning, and quantum networks. He received his M. Sc from the Department of Cybersecurity at RIT. He received his Bachelor's degree from the Department of Management Information Systems at the University of Dhaka, Bangladesh. 

\end{IEEEbiographynophoto}

% \vskip -3\baselineskip plus -1fil

\begin{IEEEbiographynophoto}{Stephen DiAdamo}
received the Dr.-Ing degree in electrical engineering from the Technical University of Munich in 2023. Currently, he is a quantum research scientist at Cisco Quantum Lab.

\end{IEEEbiographynophoto}
% \vskip -3\baselineskip plus -1fil


\begin{IEEEbiographynophoto}{Miralem Mehic} received his Ph.D. degree in telecommunications from the VSB-Technical University of Ostrava (Czechia). He is an associate professor at the Department of Telecommunications, Faculty of Electrical Engineering, University of Sarajevo, Bosnia and Herzegovina. His research interests focus on security and routing, especially security services, network management, cryptanalysis, intrusion detection, routing protocols, quality of service, steganography and quantum cryptography. 

\end{IEEEbiographynophoto}
% \vskip -3\baselineskip plus -1fil


\begin{IEEEbiographynophoto}{Charles Fleming} received a Ph.D in Computer Science at UCLA in 2013 and held professorships at Xi'an Jiaotong-Liverpool University and the University of Mississippi. Currently, he is a research scientist at Cisco. 

\end{IEEEbiographynophoto}


